Frustration solitaire

In this expository article, we discuss the rank-derangement problem, which asks for the number of permutations of a deck of cards such that each card is replaced by a card of a different rank. This combinatorial problem arises in computing the probability of winning the game of `frustration solitaire'. The solution is a prime example of the method of inclusion and exclusion. We also discuss and announce the solution to Montmort's `Probleme du Treize', a related problem dating back to circa 1708.

==> rank_dot_bib <==
@article{chungFuchs:sums,
	author =	"K. L. Chung and W. H. J. Fuchs",
	title =		"On the distribution of values of sums of random variables",
	journal =	"Mem. Amer. Math. Soc.",
	volume =	"6",
	year =		"1951"
}

@book{feynmann:lectures,
	author =	"R. P. Feynmann",
	title =		"The {F}eynmann Lectures on Physics",
	publisher =	"Addison-Wesley",
	year =		"1964"
}

@book{guivarchEtAl:marches,
	author =	"Y. Guivarc'h and M. Keane and B. Roynette",
	title =		"Marches al{\'e}atoires sur les groupes de Lie (Lecture
Notes in Math 624)",
	publisher =	"Springer",
	year =		"1977"
}

@book{hodge:harmonic,
	author =	"W. V. D. Hodge",
	title =	"The Theory and Applications of Harmonic Integrals (2nd edition",
	publisher =	"Cambridge",
	year =		"1951"
}

@book{jeans:electricity,
	author =	"J. Jeans",
	title =	"The MAthematical Theory of Electricity and Magnetism, 5th edition",
	publisher =	"Cambridge",
	year =		"1966"
}

@article{kestenGrimmett:silver,
	author =	"H. Kesten and ? Grimmett",
	title =		"Silver and gold?",
	journal =	"?",
	volume =	"?",
	year =		"?",
	pages =		"?"
}

@book{lamperti:probability,
	author =	"J. Lamperti",
	title =		"Probability:  A Survey of the Mathematical Theory",
	publisher =	"Benjamin",
	year =		"1966"
}

@article{onsager:reciprocal,
	author =	"L. Onsager",
	title =		"Reciprocal relations in irreversible processes {I}",
	journal =	"Phys. Rev.",
	volume =	"37",
	year =		"1931",
	pages =		"405-426"
}

@article{polya:irrfahrt,
	author =	"G. Polya",
	title =		"{\"{U}}ber eine {A}ufgabe betreffend die {I}rrfahrt im {S}trassennetz",
	journal =	"Math. Ann.",
	volume =	"84",
	year =		"1921",
	pages =		"149-160"
}

@article{whitney:abstract,
	author =	"H. Whitney",
	title =		"On the abstract properties of linear dependence",
	journal =	"Amer. J. Math.",
	volume =	"57",
	year =		"1935",
	pages =		"509-533"
}




@article{abikoff:uniformization,
	author =	"W. Abikoff",
	year =		"1981",
	journal =	"Amer. Math. Monthly",
	pages =		"574-592",
	title =		"The uniformization theorem",
	volume =	"88"
}

@article{ackermann:zahlen,
	author =	"W. Ackermann",
	title =		"Zum {H}ilbertschen {A}ufbau der reellen {Z}ahlen",
	journal =	"Math. Ann.",
	volume =	"99",
	year =		"1928",
	pages =		"118-133"
}

@article{ahlfors:typus,
	author =	"L. V. Ahlfors",
	year =		"1931",
	journal =	"Comment. Math. Helv.",
	pages =		"173-177",
	title =		"Zur {B}estimmung der {T}ypus einer {R}iemannschen {F}l{\"{a}}che",
	volume =	"3"
}

@article{ahlfors:ueberlagerungsflaechen,
	author =	"L. V. Ahlfors",
	year =		"1935",
	journal =	"Acta Math.",
	pages =		"157-194",
	title =		"Zur {T}heorie der {\"{U}}berlagerungsfl{\"{a}}chen",
	volume =	"65"
}

@book{ahlforsSario:riemannSurfaces,
	author =	"L. V. Ahlfors and L. Sario",
	address =	"Princeton, N. J.",
	year =		"1960",
	publisher =	"Princeton Univ. Press",
	title =		"{R}iemann Surfaces"
}

@article{ahlswedeDaykin:fkg,
	author =	"R. Ahlswede and D. E. Daykin",
	year =		"1978",
	journal =	"Z. Wahrsch. Verw. Gebiete",
	pages =		"183-185",
	title =		"An inequality for the weights of two families of sets, their unions and intersections",
	volume =	"43"
}

@article{akaza:schottky,
	author =	"T. Akaza",
	title =		"Poincar\'{e} theta-series and singular sets of {S}chottky groups",
	journal =	"Nagoya Math. J.",
	volume =	"24",
	year =		"1964",
	pages =		"43-65"
}

@article{akaza:measure,
	author =	"T. Akaza",
	title =		"(3/2)-dimensional measure of singular sets of some {K}leinian groups",
	journal =	"J. Math. Soc. Japan",
	volume =	"24",
	year =		"1972",
	pages =		"448-464"
}

@techreport{aspvallLiang:dinnerTable,
	author =	"B. Aspvall and F. M. Liang",
	title =		"The dinner table problem",
	number =	"STAN-CS-80-8222",
	institution =	"Computer Science Department, Stanford University",
	address =	"Stanford, California",
	year =		"1980"
}

@article{avez:ohp,
	author =	"A. Avez",
	title =		"Th\'{e}or\`{e}me de {C}hoquet-{D}eny pour les groupes de croissance non exponentielle",
	journal =	"C. R. Acad. Sciences Paris S\'{e}r. A",
	volume =	"279",
	year =		"1974",
	pages =		"25-28"
}

@book{bachmann:transfinite,
	author =	"H. Bachmann",
	title =		"Transfinite Zahlen (Zweite Auflage)",
	publisher =	"Springer",
	address =	"Berlin",
	year =		"1967"
}

@article{baumPetrie,
	author =	"L. E. Baum and T. Petrie",
	title =		"Statistical inference for probabilistic functions of finite state Markov chains",
	journal =	"Ann. Math. Stat.",
	volume =	"37",
	year =		"1966",
	pages =		"1554-1563"
}

@article{baumEagon,
	author =	"L. E. Baum and J. A. Eagon",
	title =		"An inequality with applications to statistical estimation for probabilistic functions of Markov processes and to a model for ecology",
	journal =	"Bull. Amer. Math. Soc.",
	volume =	"73",
	year =		"1967",
	pages =		"360-363"
}

@article{baumSell,
	author =	"L. E. Baum and G. R. Sell",
	title =		"Growth transformations for functions on manifolds",
	journal =	"Pacific J. Math.",
	volume =	"27",
	year =		"1968",
	pages =		"211-227"
}

@article{baumEtAl,
	author =	"L. E. Baum and T. Petrie and G. Soules and N. Weiss",
	title =		"A maximization technique occurring in the statistical analysis of probabilistic functions of Markov chains",
	journal =	"Ann. Math. Stat.",
	volume =	"41",
	year =		"1970",
	pages =		"164-171"
}


@incollection{baum:inequality,
	author =	"L. E. Baum",
	title =		"An inequality and associated maximization technique in statistical estimation for probabilistic functions of Markov processes",
	pages =		"1-8",
	booktitle =	"Inequalities, Vol. 3",
	publisher =	"Academic Press",
	address =	"New York",
	year =		"1972"
}

@article{bernstein:mengenlehre,
	author =	"F. Bernstein",
	title =		"Untersuchungen aus der {M}engenlehre",
	journal =	"Math. Ann.",
	volume =	"61",
	year =		"1905",
	pages =		"117-154"
}

@unpublished{blum:waffling,
	author =	"M. Blum",
	title =		"Breaking the complexity barrier with waffling programs",
	note =		"preprint"
}

@article{bogart:latin,
	author =	"K. P. Bogart",
	title =		"Counting 3-line {L}atin rectangles(?)",
	journal =	"?",
	volume =	"?",
	year =		"?",
	pages =		"?"
}


@article{bogartDoyle:menage,
	author =	"K. P. Bogart and P. G. Doyle",
	title =		"Non-sexist solution of the m\'{e}nage problem",
	journal =	"Amer. Math. Monthly",
	volume =	"93",
	year =		"1986",
	pages =		"514-518",
	note=
"On-line version available"
}

@book{bollobas:graph,
	author =	"B. Bollob\'{a}s",
	title =		"Graph Theory",
	publisher =	"Springer",
	address =	"New York",
	year =		"1979"
}

@article{bott:notices,
	author =	"R. Bott",
	year =		"1985",
	journal =	"Notices Amer. Math. Soc.",
	pages =		"152-158",
	title =		"On topology and other things",
	volume =	"32"
}

@article{bottDuffin:wang,
	author =	"R. Bott and R. J. Duffin",
	year =		"1951",
	journal =	"Bull. Amer. Math. Soc.",
	pages =		"136",
	title =		"The {W}ang algebra of networks",
	volume =	"57"
}

@article{bottDuffin:algebra,
	author =	"R. Bott and R. J. Duffin",
	year =		"1953",
	journal =	"Trans. Amer. Math. Soc.",
	pages =		"99-109",
	title =		"On the algebra of networks",
	volume =	"74"
}

@article{bottDuffin:synthesis,
	author =	"R. Bott and R. J. Duffin",
	year =		"1949",
	journal =	"J. Appl. Phys.",
	pages =		"816",
	title =		"Impedance synthesis without use of transformers",
	volume =	"20"
}

@article{bourbaki:working,
	author =	"N. Bourbaki",
	title =		"Foundations of mathematics for the working mathematician",
	journal =	"J. Symbolic Logic",
	volume =	"14",
	year =		"1949",
	pages =		"1-8"
}

@article{bouwer:graphs,
	author =	"I. Z. Bouwer",
	year =		"1970",
	journal =	"Canadian Math. Bull.",
	pages =		"231-237",
	title =		"Vertex and edge transitive, but not 1-transitive graphs",
	volume =	"13"
}

@article{brooks:schottky,
	author =	"R. Brooks",
	title =		"On the deformation theory of classical {S}chottky groups",
	journal =	"Duke Math. J.",
	volume =	"52",
	year =		"1985",
	pages =		"1009-1024"
}


@article{brooks:apollonian,
	author =	"R. Brooks",
	title =		"The spectral geometry of the {A}pollonian packing",
	journal =	"Comm. Pure Appl. Math.",
	volume =	"38",
	year =		"1985",
	pages =		"357-366"
}


@article{burnside:automorphic,
	author =	"W. Burnside",
	title =		"On a class of automorphic functions",
	journal =	"Proc. London Math. Soc.",
	volume =	"23",
	year =		"1891",
	pages =		"49-88"
}


@article{buser:riemann,
	author =	"P. Buser",
	title =		"Isospectral {R}iemann surfaces",
	journal =	"Ann. Inst. Fourier (Grenoble)",
	volume =	"36",
	year =		"1986",
	pages =		"167-192"
}

@incollection{buser:cayley,
	author =	"P. Buser",
	title =		"Cayley graphs and planar isospectral domains",
	pages =		"64-77",
	booktitle =	"Geometry and Analysis on Manifolds (Lecture Notes in Math. 1339)",
	editor =	"T. Sunada",
	publisher =	"Springer",
	year =		"1988"
}

@article{chaiken:matrixTree,
	author =	"S. Chaiken",
	year =		"1982",
	journal =	"SIAM J. Alg. Disc. Meth.",
	pages =		"319-329",
	title =		"A combinatorial proof of the all minors matrix tree theorem",
	volume =	"3"
}

@article{church:constructive,
	author =	"A. Church",
	title =		"The constructive second number class",
	journal =	"Bull. Amer. Math. Soc.",
	volume =	"44",
	year =		"1938",
	pages =		"224-232"
}

@article{churchKleene:ordinals,
	author =	"A. Church. and S. C. Kleene",
	title =		"Formal definitions in the theory of ordinal numbers",
	journal =	"Fundamenta Mathematicae",
	volume =	"28",
	year =		"1936",
	pages =		"11-21"
}

@incollection{cohen:comments,
	author =	"P. J. Cohen",
	title =		"Connents on the foundations of set theory",
	pages =		"9-15",
	booktitle =	"Axiomatic Set Theory, Proc. Symp. Pure Math. 13",
	editor =	"D. S. Scott",
	publisher =	"Amer. Math. Soc.",
	address =	"Providence",
	year =		"1971"
}


@book{constantinescuCornea:raender,
	author =	"C. Constantinescu and A. Cornea",
	address =	"Berlin",
	year =		"1963",
	publisher =	"Springer",
	title =		"Ideale {R}{\"{a}}nder {R}iemannschen {F}l{\"{a}}che"
}

@incollection{conway:knots,
	author =	"J. H. Conway",
	title =		"An enumeration of knots and links, and some of their algebraic properties",
	pages =		"329-358",
	booktitle =	"Computational Problems in Abstract Algebra",
	editor =	"J. Leech",
	publisher =	"Pergamon",
	address =	"Oxford",
	year =		"1970"
}

@incollection{conway:orbifolds,
        author =        "J. H. Conway",
        title =         "The orbifold notation for surface groups",
        pages =         "438-447",
        booktitle =     "Groups, Combinatorics and Geometry",
        editor =        "M. W. Liebeck and J. Saxl",
        publisher =     "Cambridge Univ. Press",
        address =       "Cambridge",
        year =          "1992"
}


@incollection{demilloLiptonPerlis:social,
	author =	"R. A. DeMillo and R. J. Lipton and A. J. Perlis",
	title =		"Social processes and proofs of theorems and programs",
	pages =		"206-213",
	booktitle =	"Conference Record of the Fourth ACM Symposium on Principles of Programming Languages, May 1977, Los Angeles",
	publisher =	"ACM Press",
	address =	"New York",
	year =		"1977"
}

@article{dempsterEtAl:jerk,
	author =	"A. P. Dempster and N. M. Laird and D. B. Rubin",
	title =		"Maximum likelihood from incomplete data via the EM algorithm",
	journal =	"Ann. Math. Stat.",
	volume =	"41",
	year =		"1970",
	pages =		"164-171"
}


@unpublished{doyle:seniorThesis,
	author =	"P. G. Doyle",
	title =		"On transitive graphs",
	note =		"Senior Thesis, Harvard College",
	month =		"April",
	year =		"1976"
}

@misc{doyle:latin,
	author =	"P. G. Doyle",
	title =		"The number of {L}atin rectangles",
	note=
"On-line version available"
}

@phdthesis{doyle:thesis,
	author =	"P. G. Doyle",
	title =		"Application of {R}ayleigh's short-cut method to {P}olya's recurrence problem",
	school =	"Dartmouth College",
	address =	"Hanover, N. H.",
	year =		"1982"
}

@article{doyle:speiser,
	author =	"P. G. Doyle",
	year =		"1984",
	journal =	"Bull. Amer. Math. Soc.",
	pages =		"371-377",
	title =		"Random walk on the {S}peiser graph of a {R}iemann surface",
	volume =	"11",
	note=
"On-line version available"
}

@book{doyleSnell:carus,
	author =	"P. G. Doyle and J. L. Snell",
	address =	"Washington, D. C.",
	title =		"Random Walks and Electric Networks",
	publisher =	"Mathematical Association of America",
	year =		"1984"
}

@article{duffin:extremal,
	author =	"R. J. Duffin",
	year =		"1962",
	journal =	"J. Math. Anal. Appl.",
	pages =		"200-215",
	title =		"The extremal length of a network",
	volume =	"5"
}

@article{duffin:wang,
	author =	"R. J. Duffin",
	year =		"1959",
	journal =	"Trans. Amer. Math. Soc.",
	pages =		"94-138",
	title =		"An analysis of the {W}ang algebra of networks",
	volume =	"93"
}

@incollection{duffin:models,
	author =	"R. J. Duffin",
	title =		"Electrical network models",
	pages =		"94-138",
	booktitle =	"Studies in Graph Theory",
	editor =	"D. R. Fulkerson",
	publisher =	"Mathematical Association of America",
	year =		"1975"
}

@article{duffin:lumped,
	author =	"R. J. Duffin",
	year =		"1959",
	journal =	"J. Math. Mech.",
	pages =		"793-826",
	title =		"Distributed and lumped networks",
	volume =	"8"
}

@article{duffin:rhombic,
	author =	"R. J. Duffin",
	year =		"1968",
	journal =	"J. Combin. Theory",
	pages =		"258-272",
	title =		"Potential theory on a rhombic lattice",
	volume =	"5"
}

@article{duffin:notSelfAdjoint,
	author =	"R. J. Duffin",
	year =		"1968",
	journal =	"Arch. Rational Mech. Anal.",
	pages =		"90-101",
	title =		"Estimating {D}irichlet's integral and electrical conductance for systems which are not self-adjoint",
	volume =	"30"
}

@article{feferman:arithmetization,
	author =	"S. Feferman",
	title =		"Arithmetization of metamathematics in a general setting",
	journal =	"Fundamenta Mathematicae",
	volume =	"49",
	year =		"1960",
	pages =		"35-92"
}

@article{feferman:transfinite,
	author =	"S. Feferman",
	title =		"Transfinite recursive progressions of axiomatic theories",
	journal =	"J. Symbolic Logic",
	volume =	"27",
	year =		"1962",
	pages =		"259-316"
}

@article{fefermanSpector:paths,
	author =	"S. Feferman and C. Spector",
	title =		"Incompleteness along paths in progressions of theories",
	journal =	"J. Symbolic Logic",
	volume =	"27",
	year =		"1962",
	pages =		"383-390"
}

@book{feller:v1,
	author =	"W. Feller",
	title =		"An Introduction to Probability Theory and its Applications, Vol. I",
	edition =	"Third",
	address =	"New York",
	year =		"1968",
	publisher =	"Wiley"
}

@article{fishburn:linearExtensions,
	author =	"Peter C. Fishburn",
	year =		"1984",
	journal =	"Order",
	pages =		"127-137",
	title =		"A correlational inequality for linear extensions of posets",
	volume =	"1"
}

@article{fisher:dimers,
	author =	"M. E. Fisher",
	year =		"1961",
	journal =	"Phys. Rev.",
	pages =		"1664-1672",
	title =		"Statistical mechanics of dimers on a plane lattice",
	volume =	"124"
}

@article{fkg,
	author =	"C. M. Fortuin and P. W. Kasteleyn and J. Ginibre",
	year =		"1971",
	journal =	"Comm. Math. Phys.",
	pages =		"89-103",
	title =		"Correlation inequalities for some partially ordered sets",
	volume =	"22"
}

@article{flanders:infinite,
	author =	"H. Flanders",
	title =		"Infinite Networks: {I}---resistive networks",
	journal =	"IEEE Trans. Circuit Theory",
	volume =	"18",
	year =		"1971",
	pages =		"326-331"
}

@article{flanders:infiniteGrid,
	author =	"H. Flanders",
	title =		"Infinite Networks: {II}---resistances in an infinite grid",
	journal =	"J. Math. Anal. Appl.",
	volume =	"40",
	year =		"1972",
	pages =		"30-35"
}

@incollection{foster:average,
	author =	"R. M. Foster",
	title =		"The average impedance of an electrical network",
	pages =		"333-340",
	booktitle =	"Contributions to Applied Mechanics (Reissner Anniversary Volume)",
	publisher =	"Edwards Bros.",
	address =	"Ann Arbor, Mich.",
	year =		"1949"
}

@article{foster:extension,
	author =	"R. M. Foster",
	title =		"An extension of a network theorem",
	journal =	"IRE Trans. Circuit Theory",
	volume =	"8",
	year =		"1961",
	pages =		"75-76"
}

@article{friedman:necessary,
	author =	"H. Friedman",
	title =		"On the necessary use of abstract set theory",
	journal =	"Adv. in Math.",
	volume =	"41",
	year =		"1981",
	pages =		"209-280"
}

@article{friedmanScedrov:induction,
	author =	"H. Friedman and Andrei {\v{S}}{\v{c}}edrov",
	title =		"Arithmetic transfinite induction and recursive well-orderings",
	journal =	"Adv. in Math.",
	volume =	"56",
	year =		"1985",
	pages =		"283-294"
}

@article{garsiaMilne:rogers,
	author =	"A. M. Garsia and S. C. Milne",
	title =		"A {R}ogers-{R}amanujan bijection",
	journal =	"J. Combin. Theory, Series A",
	volume =	"31",
	year =		"1981",
	pages =		"289-339"
}

@article{gass:notation,
	author =	"F. Gass",
	title =		"Constructive ordinal notation systems",
	journal =	"Math. Mag.",
	volume =	"57",
	year =		"1984",
	pages =		"131-141"
}


@article{gilbert:knots,
	author =	"E. N. Gilbert",
	year =		"1956",
	journal =	"Scripta Math.",
	pages =		"228-233",
	title =		"Knots and classes of m\'{e}nage permutations",
	volume =	"22"
}

@article{gordonWebbWolpert:drum,
	author =	"C. Gordon and D. Webb and S. Wolpert",
	title =		"One cannot hear the shape of a drum",
	journal =	"Bull. Amer. Math. Soc.",
	volume =	"27",
	year =		"1992",
	pages =		"134-138"
}

@article{gordonWebbWolpert:isospectral,
	author =	"C. Gordon and D. Webb and S. Wolpert",
	title =		"Isospectral plane domains and surfaces via {R}iemannian orbifolds",
	journal =	"Invent. Math.",
	volume =	"110",
	year =		"1992",
	pages =		"1-22"
}


@article{griffeathLiggett:nearest,
	author =	"D. Griffeath and T. M. Liggett",
	year =		"1982",
	journal =	"Ann. Probab.",
	pages =		"881-895",
	title =		"Critical phenomena for {S}pitzer's reversible nearest particle systems",
	volume =	"10"
}

@article{gromov:polynomial,
	author =	"M. Gromov",
	title =		"Groups of polynomial growth and expanding maps",
	journal =	"Inst. Hautes \'{E}tudes Sci. Publ. Math.",
	volume =	"53",
	year =		"1981",
	pages =		"53-78"
}

@book{hall:groups,
	author =	"M. Hall",
	address =	"New York",
	year =		"1959",
	publisher =	"Macmillan",
	title =		"The Theory of Groups"
}

@article{hamilton:ricci,
	author =	"R. S. Hamilton",
	year =		"1982",
	journal =	"J. Differential Geom.",
	pages =		"255-306",
	title =		"Three-manifolds of positive {R}icci curvature",
	volume =	"17"
}

@article{hersch:proposals,
	author =	"R. Hersch",
	title =		"Some proposals for reviving the philosophy of mathematics",
	journal =	"Adv. in Math.",
	volume =	"31",
	year =		"1979",
	pages =		"31-50"
}

@article{hilbert:unendliche,
	author =	"D. Hilbert",
	title =		"{\"{U}}ber das {U}nendliche",
	journal =	"Math. Ann.",
	volume =	"95",
	year =		"1926",
	pages =		"161-190"
}

@article{hilbert:naturerkennen,
	author =	"D. Hilbert",
	title =		"Naturerkennen und {L}ogik ",
	journal =	"Naturwissenschaften",
	year =		"1930",
	pages =		"950-963",
	note =		"(378-387 in hilbert:gesammelte, 3. Band)"
}


@book{hilbert:gesammelte,
	author =	"D. Hilbert",
	title =		"Gesammelte Abhandlungen",
	publisher =	"Springer",
	address =	"Berlin",
	year =		"1935"
}


@article{holland:minimum,
	author =	"C. J. Holland",
	year =		"1978",
	journal =	"Comm. Pure Appl. Math.",
	pages =		"509-519",
	title =		"A minimum principle for the principal eigenvalue for second-order linear elliptic equations with natural boundary conditions",
	volume =	"31"
}

@article{holley:fkg,
	author =	"R. Holley",
	year =		"1974",
	journal =	"Comm. Math. Phys.",
	pages =		"227-231",
	title =		"Remarks on the {FKG} inequalities",
	volume =	"36"
}

@article{holt:doyleGraph,
	author =	"D. F. Holt",
	year =		"1981",
	journal =	"J. Graph Theory",
	pages =		"201-204",
	title =		"A graph which is edge transitive but not arc transitive",
	volume =	"5"
}

@unpublished{hwangShepp:randomSubsets,
	author =	"F. K. Hwang and L. A. Shepp",
	title =		"Some inequalities concerning random subsets of a set",
	note =		"preprint"
}

@book{jech:setTheory,
	author =	"T. Jech",
	title =		"Set Theory",
	publisher =	"Academic Press",
	address =	"New York",
	year =		"1978"
}

@book{jech:choice,
	author =	"T. Jech",
	title =		"The Axiom of Choice",
	publisher =	"North-Holland",
	address =	"Amsterdam",
	year =		"1973"
}

@unpublished{joagDev:fkg,
	author =	"Kumar Joag-Dev",
	title =		"Association of matchmakers",
	note =		"widely distributed preprint"
}

@article{kac:drum,
	author =	"M. Kac",
	title =		"Can one hear the shape of a drum?",
	journal =	"Amer. Math. Monthly",
	volume =	"73",
	year =		"1966",
	pages =		""
}

@article{kasteleyn:dimer,
	author =	"P. W. Kasteleyn",
	year =		"1963",
	journal =	"J. Math. Phys.",
	pages =		"287-293",
	title =		"Dimer statistics and phase transitions",
	volume =	"4"
}

@article{kakutani:metrik,
	author =	"S. Kakutani",
	year =		"1937",
	journal =	"Proc. Imp. Acad. Tokyo",
	pages =		"89-92",
	title =		"{E}inf{\"{u}}hrung einer {M}etrik auf die {R}iemannsche {F}l{\"{a}}che und der {T}ypus der {R}iemannschen {F}l{\"{a}}che",
	volume =	"13"
}

@article{kakutani:pseudoregular,
	author =	"S. Kakutani",
	year =		"1937",
	journal =	"Japanese J. Math.",
	pages =		"375-392",
	title =		"Applications of the theory of pseudo-regular functions to the type-problem of {R}iemann surfaces",
	volume =	"13"
}

@article{kakutani:brownianMotionAndType,
	author =	"S. Kakutani",
	year =		"1949",
	journal =	"Proc. Japan Acad.",
	pages =		"138-140",
	title =		"Two-dimensional {B}rownian motion and the type problem of {R}iemann surfaces",
	volume =	"21"
}

@incollection{kakutani:randomWalkAndType,
	author =	"S. Kakutani",
	title =		"Random walk and the type problem of {R}iemann surfaces",
	pages =		"95-101",
	booktitle =	"Contributions to the theory of {R}iemann surfaces",
	publisher =	"Princeton Univ. Press",
	address =	"Princeton, N. J.",
	year =		"1953"
}

@article{kaplansky:menage,
	author =	"I. Kaplansky",
	year =		"1943",
	journal =	"Bull. Amer. Math. Soc.",
	pages =		"784-785",
	title =		"Solution of the probl\`{e}me des m\'{e}nages",
	volume =	"49"
}

@article{kaplanskyRiordan:menage,
	author =	"I. Kaplansky and J. Riordan",
	year =		"1946",
	journal =	"Scripta Mathematica",
	pages =		"113-124",
	title =		"The probl\`{e}me des m\'{e}nages",
	volume =	"12"
}

@article{kirchhoff:gleichungen,
	author =	"G. Kirchhoff",
	title =		"{U}eber die {A}ufl{\"{o}}sung der {G}leichungen,
				auf welche man bei der {U}ntersuchung
				der linearen {V}ertheilung {G}alvanischer
				{S}tr{\"{o}}me gef{\"{u}}hrt wird",
	journal =	"Ann. Phys. Chem.",
	volume =	"72",
	year =		"1847",
	pages =		"497-508"
}

@article{kleene:general,
	author =	"S. C. Kleene",
	title =		"General recursive functions of natural numbers",
	journal =	"Math. Ann.",
	volume =	"112",
	year =		"1936",
	pages =		"727-742"
}

@article{kleene:notation,
	author =	"S. C. Kleene",
	title =		"On notation for ordinal numbers",
	journal =	"J. Symbolic Logic",
	volume =	"3",
	year =		"1938",
	pages =		"150-155"
}

@article{kleene:forms,
	author =	"S. C. Kleene",
	title =		"On the forms of the prodicates in the theory of constructive ordinals",
	journal =	"Amer. J. Math.",
	volume =	"66",
	year =		"1944",
	pages =		"41-58"
}

@book{kleene:metamathematics,
	author =	"S. C. Kleene",
	title =		"Introduction to Metamathematics",
	publisher =	"Van Nostrand",
	address =	"Princeton",
	year =		"1952"
}

@misc{kohnLowe:method,
	author =	"R. V. Kohn and B. Lowe",
	note =		"personal communication"
}

@incollection{kohnVogelius:unknown,
	author =	"R. V. Kohn and M. Vogelius",
	title =		"Identification of an unknown conductivity by means of measurements at the boundary",
	pages =		"113-123",
	booktitle =	"Inverse Problems",
	editor =	"D. W. McLauglin",
	publisher =	"American Mathematical Society",
	address =	"Providence, R. I.",
	year =		"1984"
}

@article{kohnVogelius:determining,
	author =	"R. V. Kohn and M. Vogelius",
	year =		"1984",
	journal =	"Comm. Pure Appl. Math.",
	pages =		"289-298",
	title =		"Determining conductivity by boundary measurements",
	volume =	"37"
}

@unpublished{kohnVogelius:determiningII,
	author =	"R. V. Kohn and M. Vogelius",
	title =		"Determining conductivity by boundary measurements {I}{I}.  Interior results",
	note =		"preprint"
}

@incollection{kreisel:ordinal,
	author =	"G. Kreisel",
	title =		"Ordinal logics and the characterization of informal concepts of proof",
	pages =		"289-299",
	booktitle =	"Proceedings of the International Congress of Mathematicians at Edinburgh",
	publisher=	"??",
	year =		"1958"
}

@article{kreiselSchoenfieldWang:wellOrderings,
	author =	"G. Kreisel and J. Schoenfield and H. Wang",
	title =		"Number theoretic concepts and recursive well-orderings",
	journal =	"Archiv f. Math. Logik u. Grundlagen",
	volume =	"5",
	year =		"1960",
	pages =		"42-64"
}

@article{lindenbaumTarski:ensembles,
	author =	"A. Lindenbaum and A. Tarski",
	title =		"Communication sur les recherches de la th\'{e}orie des ensembles",
	journal =	"Comptes Rendus des s\'{e}ances de la Soci\'{e}t\'{e} des Sciences et des Letters de Varsovie, Classe {I}{I}{I}",
	volume =	"19",
	year =		"1926",
	pages =		"299-330"
}

@article{liu:forests,
	author =	"C. J. Liu",
	year =		"1981",
	journal =	"Proc. Amer. Math. Soc.",
	pages =		"659-662",
	title =		"Enumeration of forests in a graph",
	volume =	"83"
}

@book{lucas:nombres,
	author =	"E. Lucas",
	address =	"Paris",
	year =		"1891",
	publisher =	"Gauthier-Villars",
	title =		"Th\'{e}orie des nombres"
}

@article{lyons:criterion,
	author =	"T. J. Lyons",
	year =		"1983",
	journal =	"Ann. Probab.",
	pages =		"393-402",
	title =		"A simple criterion for transience of a reversible {M}arkov chain",
	volume =	"11"
}

@article{lyonsMckean:winding,
	author =	"T. J. Lyons and McKean, Jr., H. P.",
	year =		"1984",
	journal =	"Adv. in Math.",
	pages =		"212-225",
	title =		"Winding of the plane {B}rownian motion",
	volume =	"51"
}

@article{mckeanSullivan:thrice,
	author =	"McKean, Jr., H. P. and D. Sullivan",
	year =		"1984",
	journal =	"Adv. in Math.",
	pages =		"203-211",
	title =		"{B}rownian motion and harmonic functions on the class surface of the thrice-punctured sphere",
	volume =	"51"
}

@book{manin:logic,
	author =	"Yu. I. Manin",
	title =		"A course in Mathematical Logic",
	publisher =	"Springer",
	address =	"New York",
	year =		"1977"
}

@book{mandelbrot:fractals,
	author =	"B. Mandelbrot",
	address =	"San Francisco",
	year =		"1977",
	publisher =	"W. H. Freeman",
	title =		"Fractals: Form, Chance, and Dimension"
}

@book{mandelbrot:fractalGeometry,
	author =	"B. Mandelbrot",
	address =	"San Francisco",
	year =		"1983",
	publisher =	"W. H. Freeman",
	title =		"The Fractal Geometry of Nature"
}

@article{mandelbrot:limitSets,
	author =	"B. Mandelbrot",
	year =		"1983",
	journal =	"Math. Intelligencer",
	pages =		"9-17",
	title =		"Self-inverse fractals osculated by sigma-discs and the limit sets of {K}leinian groups",
	volume =	"5"
}

@article{mathias:bourbaki,
	author =	"A. R. D. Mathias",
	title =		"The ignorange of {B}ourbaki",
	journal =	"Math. Intelligencer",
	volume =	"14",
	year =		"1992",
	pages =		"4-13"
}

@book{maxwell:treatise,
	author =	"J. C. Maxwell",
	title =		"Treatise on Electricity and Magnetism",
	edition =	"Third",
	publisher =	"Clarendon",
	address =	"Oxford",
	year =		"1891"
}

@article{milnor:parabolicOrHyperbolic,
	author =	"J. Milnor",
	year =		"1977",
	journal =	"Amer. Math. Monthly",
	pages =		"43-46",
	title =		"On deciding whether a surface is parabolic or hyperbolic",
	volume =	"84"
}

@article{milnor:problem5603,
	author =	"J. Milnor",
	year =		"1968",
	journal =	"Amer. Math. Monthly",
	pages =		"685-686",
	title =		"Problem 5603",
	volume =	"75"
}

@article{milnor:curvatureAndFundamentalGroup,
	author =	"J. Milnor",
	year =		"1968",
	journal =	"J. Differential Geom.",
	pages =		"1-7",
	title =		"A note on curvature and fundamental group",
	volume =	"2"
}

@article{milnor:leftInvariant,
	author =	"J. Milnor",
	year =		"1976",
	journal =	"Adv. in Math.",
	pages =		"293-329",
	title =		"Curvatures of left invariant metrics on {L}ie groups",
	volume =	"21"
}

@article{milnor:affinelyFlat,
	author =	"J. Milnor",
	year =		"1977",
	journal =	"Adv. in Math.",
	pages =		"178-187",
	title =		"On fundamental groups of complete affinely flat manifolds",
	volume =	"25"
}

@article{minty:matroid,
	author =	"G. J. Minty",
	year =		"1966",
	journal =	"J. Math. Mech.",
	pages =		"485-520",
	title =		"On the axiomatic foundations of the theories of directed linear graphs, electrical networks and network-programming",
	volume =	"15"
}


@book{montmort:hazard,
	author = "de Montmort, Pierre Remand",
	title =	"Essay d'analyse sur les jeux de hazard",
	publisher =	"J. Quillau",
	address =	"Paris",
	year =		"1708"
}

@article{myrberg:konvergenzErste,
	author =	"P. J. Myrberg",
	title =		"Zur {T}heorie der {K}onvergenz der {P}oincar\'{e}schen {R}eihen",
	journal =	"Ann. Acad. Sci. Fenn. Ser. A",
	volume =	"9",
	year =		"1916",
	pages =		"1-75"
}

@article{myrberg:konvergenzZweite,
	author =	"P. J. Myrberg",
	title =		"Zur {T}heorie der {K}onvergenz der {P}oincar\'{e}schen {R}eihen (zweite Abh.)",
	journal =	"Ann. Acad. Sci. Fenn. Ser. A",
	volume =	"11",
	year =		"1917",
	pages =		"1-29"
}

@article{nashwilliams:rayleigh,
	author =	"C. St. J. A. Nash-Williams",
	year =		"1959",
	journal =	"Proc. Camb. Phil. Soc.",
	pages =		"181-194",
	title =		"Random walk and electric currents in networks",
	volume =	"55"
}

@phdthesis{nechvatal:thesis,
	author =	"J. Nechvatal",
	title =		"Counting {L}atin rectangles(?)",
	school =	"USC",
	address =	"Los Angeles, California",
	year =		"1979"
}

@book{nelson:predicative,
	author =	"E. Nelson",
	title =		"Predicative Arithmetic",
	publisher =	"Princeton University Press",
	address =	"Princeton",
	year =		"1986"
}

@book{nelson:tensor,
	author = 	"E. Nelson",
	title =		"Tensor Analysis",
	address =	"Princeton",
	year =		"1967",
	publisher =	"Princeton University Press"
}


@book{nevanlinna:eindeutige,
	author =	"R. Nevanlinna",
	address =	"Berlin",
	year =		"1953",
	publisher =	"2. Aufl., Springer",
	title =		"Eindeutige analytische {F}unktionen"
}

@article{osserman:3space,
	author =	"R. Osserman",
	year =		"1956",
	journal =	"Proc. Amer. Math. Soc.",
	pages =		"54-58",
	title =		"A hyperbolic surface in 3-space",
	volume =	"7"
}

@article{osserman:classA,
	author =	"R. Osserman",
	year =		"1956",
	journal =	"Trans. Amer. Math. Soc.",
	pages =		"217-245",
	title =		"{R}iemann surfaces of class {A}",
	volume =	"82"
}

@article{patterson:limitSet,
	author =	"S. J. Patterson",
	title =		"The limit set of a {F}uchsian group",
	journal =	"Acta Math.",
	volume =	"136",
	year =		"1976",
	pages =		"241-273"
}

@article{patterson:examples,
        author =        "S. J. Patterson",
	title =		"Some examples of {F}uchsian groups",
	journal =	"Proc. London Math. Soc.",
	volume =	"39",
	year =		"1979",
	pages =		"276-298"
}

@article{peter:nicht,
	author =	"R. P{\'{e}}ter",
	title =		"Konstruktion {N}ichtrekursiver {F}unktionen",
	journal =	"Math. Ann.",
	volume =	"111",
	year =		"1935",
	pages =		"42-60"
}

@article{phillipsSarnak:conjecture,
	author =	"R. Phillips and P. Sarnak",
	title =		"The {L}aplacian for domains in hyperbolic space and limit sets of {K}leinian groups",
	journal =	"Acta Math.",
	volume =	"155",
	year =		"1985",
	pages =		"173-241"
}

@book{pogorelov:extrinsic,
	author =	"A. V. Pogorelov",
	title =		"Extrinsic Geometry of Convex Surfaces",
	publisher = 	"American Mathematical Society",
	series = 	"Translations of Mathematical Monographs, vol. 35",
	address = 	"Providence, R.I.",
	year =		"1973"
}

@book{pogorelov:verbiegung,
	author =	"A. V. Pogorelov",
	title =		"Die {V}erbiegung konvexer {F}l{\"{a}}chen",
	publisher = 	"Akademie-Verlag",
	address = 	"Berlin",
	year =		"1957"
}

@book{protterWeinberger:maximum,
	author =	"M. H. Protter and H. F. Weinberger",
	address =	"Englewood Cliffs",
	year =		"1967",
	publisher =	"Prentice-Hall",
	title =		"Maximum principles in differential equations"
}

@incollection{rayleigh:resonance,
	author =	"J. W. S. Rayleigh",
	title =		"On the theory of resonance",
	pages =		"33-75",
	booktitle =	"Collected scientific papers",
	publisher =	"Cambridge Univ. Press",
	address =	"Cambridge",
	year =		"1899",
	volume =	"1"
}

@incollection{rayleigh:approximate,
	author =	"J. W. S. Rayleigh",
	title =		"On the approximate solution of certain problems relating to the potential",
	pages =		"??-??",
	booktitle =	"Collected scientific papers",
	publisher =	"Cambridge Univ. Press",
	address =	"Cambridge",
	year =		"1899",
	volume =	"1"
}

@article{remmel:partition,
	author =	"J. B. Remmel",
	title =		"Bijective proofs of some classical partition identities",
	journal =	"J. Combin. Theory, Series A",
	volume =	"33",
	year =		"1982",
	pages =		"273-286"
}

@book{riordan:combinatorial,
	author =	"J. Riordan",
	address =	"New York",
	year =		"1958",
	publisher =	"Wiley",
	title =		"An Introduction to Combinatorial Analysis"
}

@article{robbins:neighbors,
	author =	"D. Robbins",
	year =		"1980",
	journal =	"Amer. Math. Monthly",
	pages =		"122-124",
	title =		"The probability that neighbors remain neighbors after random rearrangements",
	volume =	"87"
}

@incollection{robinson:formalism64,
	author =	"A. Robinson",
	title =		"Formalism 64",
	pages =		"228-246",
	booktitle =	"Logic, Methodology and Philosophy of Science",
	editor =	"Y. Bar-Hillel",
	publisher =	"North-Holland",
	address =	"Amsterdam",
	year =		"1965"
}

@book{rodinSario:principal,
	author =	"B. Rodin and L. Sario",
	title =		"Principal Functions",
	publisher =	"D. van Nostrand",
	address =	"Princeton, N. J.",
	year =		"1968"
}

@article{royden:thesis,
	author =	"H. L. Royden",
	year =		"1952",
	journal =	"Trans. Amer. Math. Soc.",
	pages =		"40-94",
	title =		"Harmonic functions on open {R}iemann surfaces",
	volume =	"73"
}

@book{russell:intro,
	author =	"B. Russell",
	title =		"Introduction to Mathematical Philosophy",
	publisher =	"Allen and Unwin",
	address =	"London",
	year =		"1919"
}

@book{ryser:carus,
	author =	"H. J. Ryser",
	address =	"Washington, D. C.",
	title =		"Combinatorial Mathematics",
	publisher =	"Mathematical Association of America",
	year =		"1963"
}

@incollection{sarnak:domains,
	author =	"P. Sarnak",
	title =		"Domains in hyperbolic space and limit sets of {K}leinian groups",
	pages =		"485-500",
	booktitle =	"Differential Equations",
	editor =	"I. W. Knowles and R. T. Lewis",
	publisher =	"North-Holland",
	address =	"Amsterdam",
	year =		"1984"
}

@article{savant:frustration,
	author =	"vos Savant, Marilyn",
	title =		"Ask {M}arilyn:  {A} hat-check problem",
	journal =	"Parade Magazine",
	year =		"21 August 1994"
}

@article{schottky:specielle,
	author =	"F. Schottky",
	title =		"{\"{U}}ber eine specielle {F}unction, welche bei einer bestimmten linearen {T}ransformation ihres {A}rgumentes unver{\"{a}}ndert bleibt",
	journal =	"Crelle's J.",
	volume =	"101",
	year =		"1887",
	pages =		"227-272"
}

@article{seymourWelsh:fkg,
	author =	"P. D. Seymour and D. J. A. Welsh",
	year =		"1975",
	journal =	"Math. Proc. Cambridge Philos. Soc.",
	pages =		"485-496",
	title =		"Combinatorial applications of an inequality from statistical mechanics",
	volume =	"77"
}

@article{shepp:dubins,
	author =	"L. A. Shepp",
	title =		"Connectedness of certain random graphs",
	journal =	"Israel J. Math.",
	volume =	"67",
	year =		"1989"
}


@article{shepp:monotonicity,
	author =	"L. A. Shepp",
	year =		"1980",
	journal =	"SIAM J. Alg. Disc. Meth.",
	pages =		"295-299",
	title =		"The {FKG} inequality and some monotonicity properties of partial orders",
	volume =	"1"
}

@article{shepp:xyz,
	author =	"L. A. Shepp",
	year =		"1982",
	journal =	"Ann. Probab.",
	pages =		"824-827",
	title =		"The {XYZ} conjecture and the {FKG} inequality",
	volume =	"10"
}


@article{sierpinski:two,
	author =	"W. Sierpi\'{n}ski",
	title =		"Sur l'\'{e}galit\'{e} $2m=2n$ pour les nombres cardinaux",
	journal =	"Fund. Math.",
	volume =	"3",
	year =		"1922",
	pages =		"1-6"
}

@article{sierpinski:leq,
	author =	"W. Sierpi\'{n}ski",
	title =		"Sur l'implication $2m\leq 2n \rightarrow m \leq n$ pour les nombres cardinaux",
	journal =	"Fund. Math.",
	volume =	"34",
	year =		"1947",
	pages =		"148-154"
}

@incollection{smith:matroids,
	author =	"C. A. B. Smith",
	title =		"Electric currents in regular matroids",
	pages =		"262-284",
	booktitle =	"Combinatorics",
	editor =	"D. J. A. Welsh",
	publisher =	"Inst. of Math. and Appl.",
	address =	"Southend-on-Sea",
	year =		"1972"
}

@article{spector:recursive,
	author =	"C. Spector",
	title =		"Recursive well-orderings",
	journal =	"J. Symbolic Logic",
	volume =	"20",
	year =		"1955",
	pages =		"151-163"
}

@article{speiser:probleme,
	author =	"A. Speiser",
	year =		"1929",
	journal =	"Comment. Math. Helv.",
	pages =		"289-312",
	title =		"{P}robleme aus dem {G}ebiet der ganzen transzendenten {F}unktionen",
	volume =	"1"
}

@article{speiser:riemannscheFlaechen,
	author =	"A. Speiser",
	year =		"1930",
	journal =	"Comment. Math. Helv.",
	pages =		"284-293",
	title =		"{\"{U}}ber {R}iemannsche {F}l{\"{a}}chen",
	volume =	"2"
}

@book{spitzer:principles,
	author =	"F. Spitzer",
	title =		"Principles of Random Walk",
	edition =	"Second",
	publisher =	"Springer",
	address =	"New York",
	year =		"1976"
}

@book{strubecker:dg,
	author = 	"Karl Strubecker",
	title = 	"Differentialgeometrie, 3 vols.",
	publisher = 	"Walter de Gruyter & Co.",
	address = 	"Berlin",
	year =		"1959"
}

@article{sullivan:densityAtInfinity,
	author =	"D. Sullivan",
	year =		"1979",
	journal =	"Inst. Hautes \'{E}tudes Sci. Publ. Math.",
	pages =		"171-209",
	title =		"The density at infinity of a discrete group of hyperbolic isometries",
	volume =	"50"
}

@article{sullivan:discreteConformal,
	author =	"D. Sullivan",
	title =		"Discrete conformal groups and measurable dynamics",
	journal =	"Bull. Amer. Math. Soc.",
	volume =	"6",
	year =		"1982",
	pages =		"57-73"
}

@article{sullivan:oldNew,
        author =        "D. Sullivan",
	title =		"Entropy, {H}ausdorff measures old and new, and the limit sets of geometrically finite {K}leinian groups",
	journal =	"Acta Math.",
	volume =	"153",
	year =		"1983",
	pages =		"259-277"
}


@unpublished{sullivan:lambda,
	author =	"D. Sullivan",
	title =		"Lambda-potential theory on manifolds",
	note =		"preprint"
}

@article{sunada:isospectral,
	author =	"T. Sunada",
	title =		"Riemannian coverings and isospectral manifolds",
	journal =	"Ann. of Math.",
	volume =	"121",
	year =		"1985",
	pages =		"169-186"
}

@incollection{tait:knots,
	author =	"P. G. Tait",
	title =		"On knots, {I}, {I}{I}, {I}{I}{I}",
	pages =		"273-347",
	booktitle =	"Scientific Papers",
	publisher =	"Cambridge Univ. Press",
	address =	"Cambridge",
	year =		"1898"
}

@article{tarski:cancellation,
	author =	"A. Tarski",
	title =		"Cancellation laws in the arithmetic of cardinals",
	journal =	"Fundamenta Mathematica",
	volume =	"36",
	year =		"1949",
	pages =		"77-92"
}

@unpublished{thomassen:infinite,
	author =	"C. Thomassen",
	title =		"Resistances and currents in infinite electrical networks",
	note =		"preprint"
}

@article{thurston:poincareSymposium,
	author =	"W. P. Thurston",
	year =		"1982",
	journal =	"Bull. Amer. Math. Soc.",
	pages =		"357-381",
	title =		"Three dimensional manifolds, Kleinian groups and hyperbolic geometry",
	volume =	"6"
}

@article{touchard:menage,
	author =	"J. Touchard",
	year =		"1934",
	journal =	"C. R. Acad. Sciences Paris",
	pages =		"631-633",
	title =		"Sur un probl\`{e}me des permutations",
	volume =	"198"
}

@book{tutte:connectivity,
	author =	"W. T. Tutte",
	address =	"Toronto",
	year =		"1966",
	publisher =	"University of Toronto Press",
	title =		"Connectivity in Graphs"
}

@article{varopoulos:polya,
	author =	"N. Th. Varopoulos",
	title =		"Th\'{e}orie du potentiel sur des groupes et des vari\'{e}t\'{e}s",
	journal =	"C. R. Acad. Sciences Paris S\'{e}r. I",
	volume =	"302",
	year =		"1986",
	pages =		"203-205"
}

@article{wang:formalization,
	author =	"H. Wang",
	title =		"The formalization of mathematics",
	journal =	"J. Symbolic Logic",
	volume =	"19",
	year =		"1954",
	pages =		"241-266"
}

@article{watkins:action,
	author =	"M. E. Watkins",
	year =		"1971",
	journal =	"J. Combin. Theory",
	pages =		"95-104",
	title =		"On the action of non-abelian groups on graphs",
	volume =	"11"
}

@book{weinberg:network,
	author =	"L. Weinberg",
	title =		"Network Analysis and Synthesis",
	publisher =	"McGraw-Hill",
	address =	"New York",
	year =		"1962"
}

@book{weinberger:siam,
	author =	"H. F. Weinberger",
	title =		"Variational Methods for Eigenvalue Approximation",
	publisher =	"SIAM",
	address =	"Philadelphia",
	year =		"1974"
}

@article{weyl:mathLogic,
	author =	"H. Weyl",
	title =		"Mathematics and logic: {A} brief survey serving as preface to `{T}he {P}hilosophy of {B}ertrand {R}ussell'",
	journal =	"Amer. Math Monthly",
	volume =	"53",
	year =		"1946",
	pages =		"2-13"
}

@article{wilf:answer,
	author =	"H. Wilf",
	year =		"1982",
	journal =	"Amer. Math. Monthly",
	pages =		"289-292",
	title =		"What is an answer?",
	volume =	"89"
}

@book{wittich:neuere,
	author =	"H. Wittich",
	address =	"Berlin",
	year =		"1968",
	publisher =	"2. Aufl., Springer",
	title =		"{N}euere {U}ntersuchungen {\"{u}}ber eindeutige analytische {F}unktionen"
}

@article{zemanian:grounded,
	author =	"A. H. Zemanian",
	title =		"The characteristic-resistance method for grounded semi-infinite grids",
	journal =	"SIAM J. Math. Anal.",
	volume =	"12",
	year =		"1981",
	pages =		"115-138"
}

@article{zemanian:infinite,
	title =		"Infinite electrical networks",
	journal =	"Proc. IEEE",
	author =	"A. H. Zemanian",
	volume =	"64",
	year =		"1976",
	pages =		"6-17"
}



#
#
#  This bibliography database is atapted from Curt McMullen's as of
# 4 Dec 1987
#
@article{Abel:quintic,
	key = "Abel",
	author = "N.H. Abel",
	title = {Beweis der {U}nm{\"o}glichkeit algebraische 
		{G}leichungen von h{\"o}heren {G}raden als dem 
		vierten allgemein aufzul{\"o}sen},
	journal = "J. reine u. Angew. Math.",
	volume="1",year="1826", pages="65-84"}

@article{Abikoff:bdry,
	key="Ab",
	author="W. Abikoff",
	title={On boundaries of {T}eichm{\"u}ller spaces and
		on {K}leinian groups:  {I}{I}{I}},
	journal="Acta Math.",volume="134",
	year="1975",pages="211-237"}

@article{Abikoff:degenerating,
	key="Ab",
	author="W. Abikoff",
	title={Degenerating families of {R}iemann surfaces},
	journal="Annals of Math.",volume="105",
	year="1977",pages="29-44"}
	 
@article{Ahlfors:finiteness,
	key = "Ah",
	author = "L. Ahlfors",
	title = "Finitely generated {K}leinian groups",
	journal = "Amer. J. of Math.",
	volume="86",year="1964",pages="413-429"}

@article{Ahlfors:visual,
	key = "Ah",
	author = "L. Ahlfors",
	title = "Invariant operators and integral representations
		in hyperbolic space",
	journal = "Math. Scan.",
	volume="36",year="1975",pages="27-43"}

@article{Ahlfors:qcdef,
	key = "Ah",
	author = "L. Ahlfors",
	title = "Quasiconformal defomrations and mappings in $R^n$",
	journal = "J. d'Analyse Math.",
	volume="30",year="1976",pages="74-97"}

@incollection{Ahlfors:somewhat,
	key="Ah",
	author = "L. Ahlfors",
	title = "A somewhat new approach to quasiconformal mappings
		in $R^n$",
	booktitle="Complex Analysis",
	publisher="Springer-Verlag Lecture Notes in Math. 599",
	year="1977"}

@article{Ahlfors:Bers,
	key = "AB",
	author = "L. Ahlfors and L. Bers",
	title = "{R}iemann's mapping theorem for
		variable metrics",
	journal = "Annals of Math.",
	volume = "72", year = "1960", pages = "385-404"}

@article{Arnold:braids,
	key = "Arn",
	author = "V. I. Arnold",
	title = "On some topological invariants of 
		algebraic functions",
	journal = "Trans. Moscow Math. Soc.",
	volume="21",year="1970",pages="30-52"}

@article{Arnold:compose,
	key = "Arn",
	author = "V. I. Arnold",
	title = "Topological invariants of algebraic functions. {I}{I}",
	journal = "Func. Anal. \& Appl.",
	volume="4",year="1970",pages="91-99"}

@book{Baily:book,
	key = "Ba",
	author = "W. Baily",
	title =  "Introductory Lectures on Automorphic Forms",
	publisher ="Princeton University Press", year ="1973"}

@book{Beardon:book,
	key= "Bea",
	author= "A. Beardon",
	title= "The Geometry of Discrete Groups",
	publisher= "Springer-Verlag",year="1983"}

@article{Bers:simunif,
	key = "Bers",
	author = "L. Bers",
	title = "Simultaneous uniformization",
	journal = "Bull. AMS",
	volume="66",year="1960",pages="94-97"}

@article{Bers:schwarzian,
	key = "Bers",
	author = "L. Bers",
	title = "A non-standard integral equation with
		applications to quasiconformal mappings",
	journal = "Acta Math.",volume="116",year="1966",
	pages = "113-134"}

@article{Bers:area,
	key = "Bers",
	author = "L. Bers",
	title = "Inequalities for finitely generated 
		{K}leinian groups",
	journal = "J. d'Analyse Math.",
	volume = "18",year="1967",pages="23-41"}
	
#Contains (Thm 3) length inequality (w/slight error).
@article{Bers:bdry,
	key = "Bers",
	author = "L. Bers",
	title = {On boundaries of {T}eichm{\"u}ller spaces
		and on kleinian groups: I},
	journal = "Annals of Math.",
	volume = "91",year="1970",pages="570-600"}

@incollection{Bers:def,
	key = "Bers",
	author = "L. Bers",
	title = "Spaces of {K}leinian groups",
	booktitle = "Several Complex Variables I, Maryland 1970",
	publisher="Springer Lecture Notes in Math. 155",
	year="1970",pages="9-34"}

@article{Bers:London:survey,
	key = "Bers",
	author = "L. Bers",
	title = "Uniformization, moduli and {K}leinian groups",
	journal = "Bull. London Math. Soc.",volume="4",
	year="1972",pages="257-300"}

@incollection{Bers:nodes, 
	key = "Bers",
	author = "L. Bers",
	title =  "Spaces of degenerating {R}iemann surfaces",
	booktitle = "Discontinuous groups and {R}iemann surfaces",
	publisher = "Annals of Math Studies 76,
		Princeton University Press ",
	year="1974",
	pages="43-55"}

@article{Bers:qc:survey,
	key="Bers",
	author="L. Bers",
	title="Quasiconformal mappings, with applications
	to differential equations, function theory and
	topology",
	journal="Bull. AMS",
	volume="83",year="1977",pages="1083-1100"}

@article{Bers:mcg,
	key = "Bers",
	author = "L. Bers",
	title = "An extremal problem for quasiconformal maps
		and a theorem by {T}hurston",
	journal = "Acta Math.",
	volume = "141",year="1978",pages="73-98"}

@article{Bers:ts:survey,
	key = "Bers",
	author = "L. Bers",
	title = {Finite dimensional {T}eichm{\"u}ller spaces
		and generalizations},
	journal = "Bull. AMS",
	volume = "5",year="1981",pages="131-172"}

@article{Bers:families,
	key = "Bers",
	author = "L. Bers",
	title = {Holomorphic families of isomorphisms
		of {M}{\"o}bius groups},
	journal = "J. of Math. of Kyoto University",
	volume = "26", year="1986", pages="73-76"}

@article{Bers:Royden,
	key = "BR",
	author = "L. Bers and H. L. Royden",
	title = "Holomorphic families of injections",
	journal = "Acta Math.",
	volume="157",year="1986",pages="259-286"}

@article{BH:tracks,
	key="BH",
	author="M. Bestvina and M. Handel",
	title="Train tracks and automorphisms of free groups",
	journal="Preprint"}

@article{Bonahon:tame,
	key="Bon",
	author="F. Bonahon",
	title="Bouts des vari{\'e}t{\'e}s hyperboliques de
		dimension 3",
	journal="Annals of Math.",
	volume="124",year="1986",pages="71-158"}

@article{Bonatti:commuting,
	key="Bon",
	author="C. Bonatti",
	title="Un point fixe commun pour des 
	diff{\'e}omorphismes commutants de $S^2$",
	journal="Annals of Math.",
	volume="129",year="1989",pages="61-69"}

@article{Branner:Douady,
	key = "BD",
	author="B. Branner and A. Douady",
	title="Surgery on complex polynomials",
	booktitle="Holomorphic Dynamics",
	publisher="Springer-Verlag Lecture Notes in Math. 1345",
	year="1988"}

@book{Brocker:Dieck,
	key="BD",
	author={T. Br{\"o}cker and T. tom Dieck},
	title = "Representations of Compact {L}ie Groups",
	publisher="Springer-Verlag",year="1985"}

@article{Brooks:amenable,
	key = "Br",
	author  ="R. Brooks",
	title   ="The fundamental group and the spectrum of the Laplacian",
	journal ="Comment. Math. Helv.",
	volume ="56", year="1985", pages="581-596"}

@article{Chabauty:compactness,
	key = "Cha",
	author = "C. Chabauty",
	title = "Limites d'ensembles et g{\'e}ometrie des 
		nombers",
	journal = "Bull. Soc. Math. de France",
	volume = "78", year = "1950", pages = "143-151"}

@article{CV:graphs,
	key="CV",
	author="M. Culler and K. Vogtmann",
	title="Moduli of graphs and automorphisms 
		of free groups",
	journal="Invent. math.",volume="84",
	year="1986",pages="91-119"}

@article{Deligne:Mumford,
	key = "DM",
	author	="P. Deligne and D. Mumford",
	title 	="The irreducibility of the space of curves of given genus",
	journal ="Publications Math{\'e}matiques de l'IHES",
	volume  ="36", year="1969",pages="75-110"}

@book{Dickson:icos,
	key = "Dic",
	author = "L. Dickson",
	title = "Modern algebraic theories",
	publisher = "Benj. H. Sanborn \& Co.",
	year = "1930"}

@article{Douady:Earle,
	key = "DE",
	author = "A. Douady and C. J. Earle",
	title = "Conformally natural extension of
		homeomorphisms of the circle",
	journal = "Acta Math.",
	volume="157",year="1986",pages="23-48"}

@article{DH:polylike,
	key = "DH",
	author = "A. Douady and J. Hubbard",
	title = "On the dynamics of polynomial-like mappings",
	journal = "Ann. Sci. {\'E}c. Norm. Sup.",
	volume = "18",year="1985",pages="287-344"}

@book{DH:Orsay,
	key = "DH",
	author = "A. Douady and J. Hubbard",
	title = "{\'E}tude dynamique des polyn{\^o}mes complexes",
	publisher = "Pub. Math. d'Orsay",
	year = "1984"}

@article{DH:Thurston,
	key = "DH",
	author = "A. Douady and J. Hubbard",
	title = "A proof of {T}hurston's topological 
		characterization of rational maps",
	journal = "Institute Mittag-Leffler preprint, 1985"}

@article{Earle:theta,
	key = "Earle",
	author  ="C. J. Earle",
	title   ="Some remarks on {P}oincar{\'e} series",
	journal ="Comp. Math.",volume="21",year="1969",pages="167-176"}

@article{Earle:visual,
	key = "Earle",
	author = "C.J. Earle",
	title = "Conformally natural extension of vector fields from
		$S^{n-1}$ to $B^n$",
	journal = "Proceddings of the AMS",
	volume="102",year="1988",pages="145-149"}

@article{Earle:Marden,
	key = "EM",
	author = "C.J. Earle and A. Marden",
	title = {Geometric complex coordinates for {T}eichm{\"u}ller space},
	journal = "In preparation"}

%  Essentially inaccessible.
@incollection{Ehrenpreis:holes,
	key="Ehr",
	author="L.Ehrenpreis",
	title="Holes in moduli spaces",
	booktitle="Proceedings of the conference on quasiconformal
	mappings, moduli and discontinuous groups",
	publisher="Tulane Univ.",year="1965",pages="30-38"}

@article{Epstein:univalent,
	key = "Ep",
	author = "C. L. Epstein",
	title = "Univalence criteria and surfaces in
		hyperbolic space",
	journal = "J. reine angew. Math.",
	volume = "380",year="1987",pages="196-214"}

@book{FLP,
	key = "FLP",
	author = "A. Fathi and F. Laudenbach and V. Po{\'e}naru",
	title = "Travaux de {T}hurston sur les surfaces",
	publisher = "Asterisque",
	volume = "66-67",year="1979"}

@article{Freedman:He:spiral,
	key = "FH",
	author = "M.H. Freedman and Z.-X. He",
	title = "Factoring the logarithmic spiral",
	journal = "Invent. math.",
	volume = "92",year="1988",pages="129-138"}

@book{Fricke:algebra,
	key = "Fri",
 	author = "R. Fricke",
 	title = "Lehrbuch der {A}lgebra",
	volume = "2",
 	publisher = "Vieweg", year = "1926"}
 
@article{Gamelin:corona,
	key="Gam",
	author="T. W. Gamelin",
	title = "Localization of the corona problem",
	journal = "Pacific J. Math",
	volume="34",year="1970",pages="73"}

@book{Gardiner:book,
	key = "Gar",
	author  ="F. Gardiner",
	title   ={{T}eichm{\"u}ller Theory and Quadratic Differentials},
	publisher ="Wiley Interscience", year =	"1987"}

@article{Gardiner:theta,
	key = "Gar",
	author = "F. Gardiner",
	title = "Schiffer's interior variation and quasiconformal mapping",
	journal="Duke J. Math.",volume="42",year="1975",pages="371-380"}

@book{Garnett:book,
	key="Garn",
	author="J. B. Garnett",
	title = "Bounded Analytic Functions",
	publisher="Academic Press",year="1981"}

@article{Garnett:Jones:corona,
	key="GJ",
	author="J. B. Garnett and P. W. Jones",
	title = "The corona theorem for {D}enjoy domains",
	journal="Acta Mathematica",
	volume="155",year="1985",pages="27"}

@article{Gehring:rings,
	key="Geh",
	author="F. W. Gehring",
	title="Rings and quasiconformal mappings in space",
	journal="Trans. AMS",volume="103",
	year="1962",pages="353-393"}

@incollection{Gehring:icm:86,
	key="Geh",
	author="F. W. Gehring",
	title="Topics in quasiconformal mappings",
	booktitle = "Proceedings of the International
		Conference of Mathematicians",
	year = "1986",pages = "62-80",
	publisher = "American Math. Soc."}

@article{Green:icos,
	key = "Green",
	author = "M. Green",
	title = "On the analytic solution of the equation of
		fifth degree",
	journal="Compositio Math.",volume="37",year="1978",
	pages="233-241"}

@article{Groth:BrI,
	key = "Gro",
	author="A. Grothendieck",
	title="Le groupe de {B}rauer {I}:  Alg{\`e}bres d'{A}zumaya et
		interpretations diverses",
	journal="S{\'e}m. Bourbaki",
	volume="290",year="1965"}

@article{Groth:BrII,
	key = "Gro",
	author="A. Grothendieck",
	title="Le groupe de {B}rauer {I}{I}:  Th{\'e}orie cohomologique.",
	journal="S{\'e}m. Bourbaki",
	volume="297",year="1965"}

@book{Greenleaf,
	key = "Gre",
	author ="F. P. Greenleaf",
	title 	="Invariant Means on Topological Groups",
	publisher ="Van Nostrand",year ="1969"}

@book{Gromov:book,
	key = "Grom",
	author ="M. Gromov",
	title = "Structures m{\'e}triques pour les vari{\'e}t{\'e}s
		riemanniennes",
	publisher ="CEDIC, Textes math{\'e}matiques", year="1981"} 

@article{Hamilton:condition,
	key = "Ham",
	author ="R. S. Hamilton",
	title  ="Extremal quasiconformal mappings with 
		 prescribed boundary values",
	journal ="Trans. AMS",volume="138",year="1969",pages="399-406"}

@incollection{Harvey:compactness,
	author = "W. J. Harvey",
	key="Har",
	title = "Spaces of discrete groups",
	booktitle = "Discrete Groups and Automorphic Forms",
	publisher = "Academic Press",
	year = "1977",pages="295-348"}

@incollection{Hejhal:twists,
	author = "D. A. Hejhal",
	key="Hej",
	title = "Regular b-groups and repeated {D}ehn twists",
	booktitle = "Complex Analysis, Joensuu 1987",
	publisher = "Springer-Verlag Lecture Notes in Math. 1351",
	year = "1988",pages="169-192"}

@book{Helgason:gaga,
	key="Hel",
	author="S. Helgason",
	title="Groups and Geometric Analysis",
	publisher="Academic Press",year="1984"}

@book{Hempel:book,
	key = "Hem",
	author = "J. Hempel",
	title = "3-Manifolds",
	publisher = "Annals of Math Studies 86,
		Princeton University Press",
	year = "1976"}

@book{Hocking:Young,
	key = "HY",
	author ="J.G. Hocking and G.S. Young",
	title =	"Topology",
	publisher ="Addison-Wesley", year ="1961"}

@book{Jaco:Shalen,
	key = "JS",
	author = "W. Jaco and P. Shalen",
	title = "{S}eifert fibered spaces in 3-manifolds",
	publisher = "Memoirs of the AMS, No. 220",
	year = "1979"}

@article{John:Nirenberg,
	key="JN",
	author="F. John and L. Nirenberg",
	title ="On functions of bounded mean oscillation",
	journal="Comm. Pure App. Math.",
	volume="14",year="1961",pages="415-426"}

@article{Kazhdan:Margulis,
	key="KM",
	author="D. A. Kazhdan and G. A. Margulis",
	title ="A proof of {S}elberg's conjecture",
	journal="Math. USSR -- Sbornik",
	volume="4",year="1968",pages="147-152"}

@article{Kerckhoff:Thurston,
	key="KT",
	author="S. Kerckhoff and W. Thurston",
	title={Non-continuity of the action of the modular group at
		{B}ers' boundary of {T}eichm{\"u}ller space},
	journal="Preprint" }

@book{Klein:elem,
	key = "Klein",
	author = "F. Klein",
	title = "Elementary mathematics from an advanced
		standpoint.  Arithmetic, Algebra, Analysis",
	publisher = "McMillan Co.",year="1932"}

@book{Klein:icos,
	key = "Klein",
	author = "F. Klein",
	title = {Vorlesungen {\"u}ber das {I}kosaeder und die
		{A}ufl{\"o}sung der {G}leichungen vom f{\"u}nften {G}rade},
	publisher = "B.G. Teubner",year="1884"}

@book{Klein:vol2,
	key = "Klein",
	author = "F. Klein",
	title="Gesammelte Mathematische Abhandlungen",
	volume = "2",
	publisher="Springer",year="1922"}

# Frobenius reciprocity:  theorem 1.14
@book{Knapp:book,
	key="Kn",
	author="A. W. Knapp",
	title="Representation Theory of Semisimple Groups",
	publisher="Princeton University Press",year="1986"}

@book{Kra:book,
	key = "Kra",
	author = "I. Kra",
	title  = "Automorphic Forms and {K}leinian Groups",
	publisher ="W.A. Benjamin, Inc.", year ="1972"}

@article{Krushkal:starlike,
	key="Kru",
	author="S. L. Krushka{\'l}",
	title={On the question of the structure of the universal
		{T}eichm{\"u}ller space},
	journal="Sov. Math. Dokl.",volume="38",year="1989",
	pages="435-437"}

@incollection{Kra:def,
	key = "Kra",
	author ="I. Kra",
	title =	"Deformation spaces",
	booktitle = "A Crash Course on {K}leinian Groups",
	publisher = "Springer-Verlag Lecture Notes 400",
	pages="48-70", year = "1974"}

@article{Kra:survey,
	key = "Kra",
	author ="I. Kra",
	title =	{Canonical mappings between {T}eichm{\"u}ller spaces},
	journal="Bull. AMS", 
  	volume="4",year="1981", pages="143-179"}

#Has Hadamard 3 circles theorem.
@book{Lang:complex_analysis,
	key = "Lang",
	author = "S. Lang",
	title = "Complex Analysis",
	publisher="Springer-Verlag",year="1985"}

@book{Lehto:Virtanen,
	key = "LV",
	author = "O. Lehto and K.J. Virtanen",
	title = "Quasiconformal Mappings in the Plane",
	publisher = "Springer-Verlag",year="1973"}

#  Destroying positive harmonic functions. 
@article{Lyons:positive,
	key = "Lyons",
	author = "T. Lyons",
	title = "Instability of the {L}iouville property
		for quasi-isometric {R}iemannian manifolds
		and reversible {M}arkov chains",
	journal = "J. Diff. Geom.",
	volume="26",year="1987",pages="33-66"}

@article{Lyons:Sullivan,
	key = "LS",
	author ="T. Lyons and D. Sullivan",
	title  ="Function theory, random paths and covering spaces",
	journal="J. Diff. Geom.",volume="19",year="1984",pages="299-323"}

@article{Lyubich:typical,
	key = "Lyu",
	author = "M. Yu. Lyubich",
	title = "On typical behavior of the trajectories
		of a rational mapping of the sphere",
	journal = "Soviet Math. Dokl.",
	volume = "27",year="1983",pages="22-25"}

@article{ManeSS,
	key = "MSS",
	author = "R. Ma\~ne and P. Sad and D. Sullivan",
	title = "On the dynamics of rational maps",
	journal = "Ann. Sci. {\'E}c. Norm. Sup.",
	volume = "16",year="1983",pages="193-217"}

@article{Marden:kgs,
	key = "Mar",
	author="A. Marden",
	title ="The geometry of finitely generated 
		kleinian groups",
	journal = "Annals of Math.",
	volume = "99",year="1974",pages="383-462"}

@incollection{Marden:NATO,
	key="Mar",
	author="A. Marden",
	title="Geometrically finite {K}leinian groups and their
	deformation spaces",
	booktitle="Discrete groups and automorphic functions",
	publisher="Academic Press",year="1977",pages="259-293"}

@article{Marden:survey,
	key = "Mar",
	author="A. Marden",
	title ="Geometric relations between homeomorphic {R}iemann surfaces",
	journal = "Bull. AMS",
	volume = "3",year="1980",pages="1001-1017"}

@article{Maskit:bdry,
	key = "Mask",
	author = "B. Maskit",
	title = {On boundaries of {T}eichm{\"u}ller spaces
		and on kleinian groups: {I}{I}},
	journal = "Annals of Math.",
	volume = "91",year="1970",pages="607-639"}

@article{Maskit:def,
	key = "Mask",
	author = "B. Maskit",
	title="Self mappings of {K}leinian groups",
	journal="Amer. J. Math.",
	volume="93",year="1971",pages="840-856"}

@article{Masur:WP,
	key = "Masur",
	author = "H. Masur",
	title = {On a class of geodesics in {T}eichm{\"u}ller space},
	journal="Annals of Math.",volume="102",year="1975",pages="205-221"}

@article{Masur:WP,
	key = "Masur",
	author = "H. Masur",
	title = {The extension of the {W}eil-{P}etersson metric
		to the boundary of {T}eichm{\"u}ller space},
	journal="Duke Math. J.",volume="43",year="1976",pages="623-635"}

@article{McMullen:carpets,
	key = "Mc",
	author ="C. McMullen",
	title  ="{H}ausdorff dimension of general 
		Sierpinski carpets",
	journal="Nagoya J. of Math.",
	volume="96",year="1984",pages="1-9"}

@article{McMullen:families,
	key = "Mc",
	author ="C. McMullen",
	title  ="Families of rational maps and iterative
		root-finding algorithms",
	journal="Annals of Math.",
	volume="125",year="1987",pages="467-493"}

@article{McMullen:area,
	key = "Mc",
	author ="C. McMullen",
	title =	"Area and {H}ausdorff dimension of {J}ulia sets
			of entire functions",
	journal ="Trans. AMS",
	volume ="300",year="1987",pages="329-342"}

@inproceedings{McMullen:aut,
	key = "Mc",
	author ="C. McMullen",
	title  ="Automorphisms of rational maps",
	pages = "31-60",
	booktitle ="Holomorphic Functions and Moduli I",
	publisher="Springer-Verlag",
	year =	"1988"}

@inproceedings{Earle:McMullen,
	key = "EM",
	author ="C. Earle and C. McMullen",
	title  ="Quasiconformal isotopies",
	booktitle ="Holomorphic Functions and Moduli I",
	publisher="Springer-Verlag:  MSRI publications
	volume 10",
	pages="143-154",
	year =	"1988"}

@article{McMullen:braid,
	key = "Mc",
	author ="C. McMullen",
	title  ="Braiding of the attractor and the failure
			of iterative algorithms",
	journal="Invent. math.",
	volume="91",year="1988",pages="259-272"}

@article{Doyle:McMullen,
	key = "DMc",
	author="P. Doyle and C. McMullen",
	title="Solving the quintic by iteration",
	journal="To appear, Acta Math." }

@article{McMullen:amenable,
	key = "Mc",
	author="C. McMullen",
	title={Amenability, {P}oincar{\'e} series and quasiconformal maps},
	journal="Invent. Math.",year="1989",volume="97",pages="95-127"}

@article{McMullen:iter,
	key = "Mc",
	author="C. McMullen",
	title= {Iteration on {T}eichm{\"u}ller space},
	journal="To appear, Invent. Math."}

@article{McMullen:nyas,
	key = "Mc",
	author="C. McMullen",
	title= "{R}iemann surfaces and the geometrization 
		of 3-manifolds",
	journal="Submitted to the
		Annals of the New York Academy of Sciences"}

@article{McMullen:cusps,
	key = "Mc",
	author="C. McMullen",
	title= "Cusps are dense",
	journal="Preprint"}

@article{Brooks:Eliashberg:McMullen,
	key = "BEM",
	author="R. Brooks and Y. Eliashberg and C. McMullen",
	title= "The spectral geometry of flat disks",
	journal="Preprint"}

@article{Merkurev:Suslin,
	key = "MS",
	author="A. S. Merkurev and A. A. Suslin",
	title="K-cohomology of {S}everi-{B}rauer varieties and
		the norm residue homomorphisms",
	journal="Math. USSR Izv.",volume="21",year="1983",
	pages="307-340"}

@article{Milman:reflex,
	key = "Mil",
	author ="D. P. Milman",
	title  ="On some criteria for the regularity of spaces of type ({B})",
	journal ="Dokl. Akad. Nauk SSSR (N.S.)",
	volume ="20",year="1938",pages="243-246"}

@incollection{Morgan:uniformization,
	key = "Mor",
	author = "J. Morgan",
	title = "On {T}hurston's uniformization theorem for 
		three dimensional manifolds",
	booktitle = "The Smith Conjecture",
	pages="37-125",
	publisher = "Academic Press", year = "1984"}

@article{Morgan:Shalen:I,
	key = "MS",
	author = "J. Morgan and P. Shalen",
	title = "Valuations, trees, and degenerations of
		hyperbolic structures, {I}",
	journal = "Annals of Math.",
	volume = "120",year="1984",pages="401-476"}

@incollection{Morgan:Shalen:survey,
	key = "MS",
	author = "J. Morgan and P. Shalen",
	title = "An introduction to compactifying spaces of
		hyperbolic structures by actions on trees",
	booktitle = "Geometry and Topology",
	publisher = "Springer-Verlag Lecture Notes 1167",
	year = "1985",pages="228-240"}

@article{Morita:surfaces,
	key = "Mor",
	author="S. Morita",
	title="Characteristic classes of surfaces bundles",
	journal="Invent. Math.",
	volume="90",year="1987",pages="551-577"}

@book{Mostow:book,
	author="D. Mostow",
	title="Strong rigidity of locally symmetric spaces",
	publisher="Annals of Math Studies 78, 
		Princeton University Press",
	year="1972"}

@article{Mumford:compact,
	key = "Mum",
	author ="D. Mumford",
	title  ="A remark on {M}ahler's compactness theorem", 
	journal ="Proc. AMS",volume ="28",year="1971",pages="289-294"}

@article{Nadel:levels,
	key="Nad",
	author="A. M. Nadel",
	title="The nonexistence of certain level structures
	on abelian varieties over complex function fields",
	journal="Annals of Math.",
	volume="129",year="1989",pages="161-178"}

@article{Nehari:schwarzian,
	key = "Neh",
	author = "Z. Nehari",
	title = "Schwarzian derivatives and schlicht functions",
	journal = "Bull. AMS",
	volume="55",year="1949",pages="545-551"}

@article{Ohtake:theta,
	key = "Oh",
	author = "H. Ohtake",
	title = "Lifts of extremal quasiconformal mappngs
		of arbitrary {R}iemann surfaces",
	journal = "J. Math. Kyoto Univ.",
	volume="22",year="1982",pages="191-200"}

@article{Pansu:carnot,
	key="Pan",
	author="P. Pansu",
	title="M{\'e}triques de {C}arnot-{C}arath{\'e}odory et
	quasiisom{\'e}tries des espaces sym{\'e}triques de
	rang un",
	journal="Annals of Math.",
	volume="129",year="1989",pages="1-60"}

@incollection{Parson:Sheingorn:theta1,
	key = "PS",
	author = "L.A. Parson and M. Sheingorn",
	title = "Bounding the norm of the {P}oincar{\'e} 
		$\theta$-operator",
	booktitle = "Analytic Number Theory",
	publisher = "Springer-Verlag Lecture Notes 899",
	year = "1981"}

@article{Parson:Sheingorn:theta2,
	key = "PS",
	author = "L.A. Parson and M. Sheingorn",
	title = "Exponential sums connected with 
		{R}amanujan's function $\tau(n)$",
	journal="Mathematika",
	year="1982",volume="29",pages="270-277"}

@article{Penner:pseudoAnosov,
	key="Pen",
	author="R. Penner",
	title ="A construction of pseudo-{A}nosov homeomorphisms",
	journal="Trans. AMS",volume="310",year="1988",pages="179-198"}

@article{Pettis:reflex,
	key = "Pet",
	author ="B. J. Pettis",
	title  ="A proof that every uniformly convex space is reflexive",
	journal ="Duke Math. J.", volume ="5",year="1939",pages="249-253" }

@book{Pier,
	key = "Pier",
	author ="J. P. Pier",
	title  ="Amenable Locally Compact Groups",
	publisher ="Wiley Interscience", year ="1984"}

@article{Poincare:fuchsian,
	key = "Poin",
	author ="H. Poincar{\'e}",
	title = "M{\'e}moire sur les fonctions {F}uchsiennes",
	journal ="Acta Math.",volume="1", year ="1882/3",pages="193-294"}

@incollection{Reich:Strebel,
	key = "RS",
	author ="E. Reich and K. Strebel",
	title  ="Extremal quasiconformal mappings with given boundary values",
	booktitle ="Contributions to Analysis", 
	publisher ="Academic Press", year ="1974" }

@article{Reimann:BMO,
	key = "Reim",
	author ="H.M. Reimann",
	title = "Functions of bounded mean oscillation
		and quasiconformal mappings",
	journal ="Comment. Math. Helv.",
	volume ="49",year ="1974",pages ="260-276"}

@article{Reimann:ode,
	key = "Reim",
	author ="H.M. Reimann",
	title = "Ordinary differential equations and quasiconformal mappings",
	journal ="Invent. math",
	volume="33",year="1976",pages="247-270"}

@article{Reimann:visual,
	key = "Reim",
	author ="H.M. Reimann",
	title = "Invariant extension of quasiconformal deformations",
	journal ="Ann. Acad. Sci. Fen.",
	volume="10",year="1985",pages="477-492"}

@article{Reshetnyak:liouville,
	key="Res",
	author="Yu. G. Reshetnyak",
	title="{L}iouville's theorem on conformal mappings under
		minimal regularity assumptions",
	journal="Sibirsk. Mat. Zh.",volume="8",
	year="1967",pages="835-840"}

@article{Reshetnyak:extremals,
	key="Res",
	author="Yu. G. Reshetnyak",
	title="Mappings with bounded deformation as extremals of
		{D}irichlet type integrals",
	journal="Sibirsk. Mat. Zh.",volume="9",
	year="1968",pages="487-498"}

@article{Reshetnyak:stability,
	key="Res",
	author="Yu. G. Reshetnyak",
	title="Stability estimates in {L}iouville's theorem and
		the $L^p$-integrability of the derivatives of
		quasiconformal mappings",
	journal="Sibirsk. Mat. Zh.",volume="17",
	year="1976",pages="868-896"}

@incollection{Royden:metric,
	key = "Roy",
	author = "H.L. Royden",
	title = "Automorphisms and isometries of
		{T}eichm{\"u}ller space",
	pages="369-384",
	booktitle = "Advances in the Theory of 
		{R}iemann Surfaces",
	publisher = "Princeton University Press",
	year = "1971"}

@article{Rosenblatt,
	key = "Ros",
	author ="J. M. Rosenblatt",
	title  ="A generalization of Folner's condition",
	journal="Math. Scand.", volume ="33", year ="1973", pages="153-170" }

@article{Scott:LERF,
	key = "Scott",
	author = "P. Scott",
	title = "Subgroups of surface groups are almost geometric",
	journal = "J. London Math. Soc.",
	volume="17",year="1978",pages="555-565"}

@book{Serre:LocalFields,
	key = "Serre",
	author="J.P. Serre",
	title="Local Fields",
	publisher="Springer-Verlag",year="1979"}

@incollection{Serre:icos,
	key = "Serre",
	author="J.P. Serre",
	title="Extensions icosa{\'e}driques",
	booktitle="Oeuvres {I}{I}{I}",
	publisher="Springer-Verlag",year="1986",pages="550-554"}

@article{Shiga:regular,
	key="Shiga",
	author="H. Shiga",
	title={On analytic and geometric properties of {T}eichm{\"u}ller spaces},
	journal = "J. Math. Kyoto Univ.",
	volume="24",year="1984",pages="441-452"}

@article{Shishikura:2d-2,
	key="Shi",
	author="M. Shishikura",
	title="On the quasiconformal surgery of rational functions",
	journal = "Ann. Sci. {\'E}c. Norm. Sup.",
	volume="20",year="1987",pages="1-30"}

@article{Shub:Smale,
	key = "SS",
	author="M. Shub and S. Smale",
	title="On the existence of generally convergent algorithms",
	journal="J. of Complexity",volume="2",year="1986",
	pages="2-11"}

@article{SS:Cartan,
	key = "SS",
	author = "I.M. Singer and S. Sternberg",
	title = "The infinite groups of {L}ie and {C}artan",
	journal = "J. d'Analyze Math.",
	volume="15",year="1965",pages="1-114"}

@article{Smale:cxity,
	key = "Smale",
	author="S. Smale",
	title="On the efficiency of algorithms of analysis",
	journal="Bull. AMS",volume="13",year="1985",pages="87-121"}

@incollection{Stein:survey,
	key="Stein",
	author="E. M. Stein",
	title="Singular integrals, harmonic functions, and
	differentiability properties of functions of several variables",
	booktitle="Singular Integrals",
	publisher="AMS Symposia in Pure Math. X",
	year="1967",pages="316-335"}

@book{Stein:book:singular,
	key="Stein",
	author="E. M. Stein",
	title="Singular Integrals and Differentiability
		Properties of Functions",
	publisher="Princeton Univeristy Press",
	year="1970"}

@article{Stein:Zygmund,
	key="SZ",
	author="E. M. Stein and A. Zygmund",
	title={Boundedness of translation invariant operators
		on H{\"o}lder spaces and $L^p$-spaces},
	journal="Annals of Math.",volume="85",year="1967",
	pages="337-349"}

@book{Strebel:book,
	key = "Str",
	author ="K. Strebel",
	title  ="Quadratic Differentials",
	publisher ="Springer-Verlag", year ="1984"}

@article{Strebel:survey,
	key = "Str",
	author ="K. Strebel",
	title  ="Extremal quasiconformal mappings",
	journal="MSRI Preprint",year="1986"}

@article{Strebel:theta,
	key = "Str",
	author ="K. Strebel",
	title  ="On lifts of extremal quasiconformal mappings",
	journal="J. d'Analyse Math.",volume="31",year ="1977",pages="191-203"}

@article{Strebel:open,
	key = "Str",
	author ="K. Strebel",
	title  ="On quasiconformal mappings of open {R}iemann surfaces",
	journal="Comment. Math. Helv.",volume="53",year="1978",pages="301-321"}

@incollection{Sullivan:linefield,
	key = "Sul",
	author = "D. Sullivan",
	title = "On the ergodic theory at infinity of an
	arbitrary discrete group of hyperbolic motions",
	booktitle = "{R}iemann Surfaces and Related Topics:
	Proceedings of the 1978 Stony Brook Conference",
	publisher = "Annals of Math. Studies 97, Princeton",
	year = "1981"}

@article{Sullivan:rot_inv,
	key = "Sul",
	author = "D. Sullivan",
	title = "For $n > 3$ there is only one finitely
	additive rotationally invariant measure on the
	$n$-sphere defined on all Lebesgue measurable sets",
	journal="Bull. AMS",volume="4",year = "1981",pages="121-123"}

@article{Sullivan:disj_spheres,
	key = "Sul",
	author = "D. Sullivan",
	title = "Disjoint spheres, approximation by imaginary
	quadratic numbers, and the logarithm law for geodesics",
	journal="Acta Math.",volume="149",year = "1982",pages="215-238"}

@incollection{Sullivan:CDS,
	key = "Sul",
	author = "D. Sullivan",
	title = "Conformal dynamical systems",
	booktitle = "Geometric Dynamics",
	publisher="Springer-Verlag Lecture Notes No. 1007",
	year="1983",pages="725-752"}

@article{Sullivan:QCDI,
	key = "Sul",
	author = "D. Sullivan",
	title = "Quasiconformal homeomorphisms and
		dynamics {I}: {S}olution of the {F}atou-{J}ulia
		problem on wandering domains",
	journal="Annals of Math.",
	volume="122",year="1985",pages="401-418"}

@article{Sullivan:QCDII,
	key = "Sul",
	author = "D. Sullivan",
	title = "Quasiconformal homeomorphisms and
		dynamics {I}{I}: {S}tructural stability implies
		hyperbolicity for {K}leinian groups",
	journal="Acta Math.",
	volume="155",year="1985",pages="243-260"}

@article{Sullivan:QCDIII,
	key = "Sul",
	author = "D. Sullivan",
	title = "Quasiconformal homeomorphisms and
		dynamics {I}{I}{I}: {T}opological conjugacy classes of
		analytic endomorphisms",
	journal="Preprint"}

@incollection{Sullivan:ICM,
	key = "Sul",
	author = "D. Sullivan",
	title = "Quasiconformal homeomorphisms in dynamics,
		topology and geometry",
	booktitle = "Proceedings of the International
		Conference of Mathematicians",
	year = "1986",pages = "1216-1228",
	publisher = "American Math. Soc."}

@incollection{Sullivan:scales,
	key = "Sul",
	author = "D. Sullivan",
	title = "Differentiable structures on fractal-like
	sets, determined by intrinsic scaling functions
	on dual Cantor sets",
	booktitle = "The Mathematical Heritage of Herman
	Weyl",
	year = "1988",pages = "15-24",
	publisher = "AMS Proceedings
	of Symposia In Pure Mathematics, Volume 48"}

@article{Sullivan:Thurston,
	key = "ST",
	author = "D. Sullivan and W. P. Thurston",
	title = "Extending holomorphic motions",
	journal = "Acta Math.",
	volume="157",year="1986",pages="243-258"}

@article{Teich:onept,
	key = "Tei",
	author = {O. Teichm{\"u}ller},
	title = "Ein {V}erschiebungssatz 
		der quasikonformen {A}bbildung",
	journal = "Deutsche Math.",
	volume="7",year="1944",pages="336-343"}

@article{Thom:ratl,
	key = "Thom",
	author="R. Thom",
	title = "L'equivalence d'une fonction diff{\'e}rentiable
		et d'un polyn{\^o}me",
	journal="Topology",
	volume="3",year="1965",pages="297-307"}

@book{Thurston:book,
	key = "Th",
	author = "W. P. Thurston",
	title  = "Geometry and Topology of Three-Manifolds",
	publisher = "Princeton lecture notes", year = "1979"}

@article{Thurston:survey,
	key = "Th",
	author = "W. P. Thurston",
	title = "Three-dimensional manifolds, {K}leinian groups
		and hyperbolic geometry",
	journal = "Bull. AMS",
	volume="6",year="1982",pages="357-381"}

@incollection{Thurston:zippers,
	key = "Th",
	author = "W. P. Thurston",
	title="Zippers and univalent functions",
	booktitle="The Bierberbach conjecture",
	editor="A. Baernstein et al",
	publisher="AMS", year="1986",pages="185-197"}


@article{Thurston:hype1,
	key = "Th",
	author = "W. P. Thurston",
	title  = "Hyperbolic structures on 3-manifolds {I}:
		  {D}eformations of acylindrical manifolds",
	journal="Annals of Math.",volume="124",year="1986",pages="203-246"} 

@article{Thurston:hype2,
	key = "Th",
	author = "W. P. Thurston",
	title  = "Hyperbolic structures on 3-manifolds {I}{I}:
		  {S}urface groups and 3-manifolds which fiber over the circle",
	journal="To appear, Annals of Math."}


@article{Thurston:hype3,
	key = "Th",
	author = "W. P. Thurston",
	title  = "Hyperbolic structures on 3-manifolds {I}{I}{I}:
		  {D}eformation of 3-manifolds with incompressible boundary",
	journal="To appear, Annals of Math."}


@article{Thurston:hype4,
	key = "Th",
	author = "W. P. Thurston",
	title  = "Hyperbolic structures on 3-manifolds {I}{V}:
		  {C}onstruction of hyperbolic manifolds",
	journal="In preparation."}

@article{Thurston:rational,
	key = "Th",
	author = "W. P. Thurston",
	title = "On the combinatorics and dynamics of iterated
		rational maps",
	journal = "Preprint"}

@article{Thurston:mcg,
	key = "Th",
	author = "W. P. Thurston",
	title = "On the geometry and dynamics of 
		diffeomorphisms of surfaces",
	journal = "Bull. AMS",volume="19",year="1988",
	pages="417-432"}

@article{Tukia:Fuchsian,
	key="Tukia",
	author="P. Tukia",
	title="Homeomorphic conjugates of {F}uchsian groups",
	journal="J. reine angew. Math.",
	volume="391",year="1988",pages="1-54"}

@book{Vaisala:book,
	key="Vai",
	author={J. V{\"a}is{\"a}l{\"a}},
	title="Lectures on n-Dimensional Quasiconformal Mappings",
	publisher="Springer-Verlag Lecture Notes 229",
	year="1971"}

@book{vdW:ancient,
	key = "vdW",
	author="B. L. van der Waerden",
	title="Geometry and Algebra in Ancient Civilizations",
	publisher="Springer-Verlag",year="1983"}

@book{vdW:history,
	key = "vdW",
	author="B. L. van der Waerden",
	title="A History of Algebra: from al-{K}hwarizmi to
		{E}mmy {N}oether",
	publisher="Springer-Verlag",year="1985"}

@book{Vuorinen:book,
	key="Vuo",
	author="M. Vuorinen",
	title="Conformal Geometry and Quasiregular Mappings",
	publisher="Springer-Verlag Lecture Notes 1319",
	year="1988"}


@article{Wolpert:FN,
	key = "Wol",
	author = "S. Wolpert",
	title = "The {F}enchel-{N}ielsen deformation",
	journal = "Annals of Math.",volume="115",year="1982",pages="501-528"}

@article{Wright:tori,
	key="Wr",
	author="D. Wright",
	title={The shape of the boundary of {M}askit's embedding
	of the {T}eichm{\"u}ller space of once-punctured tori},
	journal="Preprint"}

# The Margulis constant is least for a square punctured torus.
# The shortest geodesic has length Log[(1+ Sqrt[2])^2] = Log[3+2Sqrt[2]].
@article{Yamada:margulis,
	key="Yam",
	author="A. Yamada",
	title="On {M}arden's universal constant of {F}uchsian groups",
	journal="Kodai Math. J.",
	volume="4",year="1981",pages="266-277"}

@book{Zelobenko:book,
	key="Zel",
	author="D. P. \v{Z}elobenko",
	title="Compact {L}ie Groups and their Representations",
	publisher="AMS Translations of Math. Monographs, vol. 40",
	year="1973"}

@book{Zimmer:book,
	key = "Zim",
	author = "R. Zimmer",
	title = "Ergodic Theory and Semisimple Groups",
	publisher = "Birkhauser Boston, Inc.", year="1984"}

